ACHORD: Communication-Aware Multi-Robot Coordination with Intermittent Connectivity

Communication is an important capability for multi-robot exploration because (1) inter-robot communication (comms) improves coverage efficiency and (2) robot-to-base comms improves situational awareness. Exploring comms-restricted (e.g., subterranean) environments requires a multi-robot system to tolerate and anticipate intermittent connectivity, and to carefully consider comms requirements, otherwise mission-critical data may be lost. In this paper, we describe and analyze ACHORD (Autonomous & Collaborative High-Bandwidth Operations with Radio Droppables), a multi-layer networking solution which tightly co-designs the network architecture and high-level decision-making for improved comms. ACHORD provides bandwidth prioritization and timely and reliable data transfer despite intermittent connectivity. Furthermore, it exposes low-layer networking metrics to the application layer to enable robots to autonomously monitor, map, and extend the network via droppable radios, as well as restore connectivity to improve collaborative exploration. We evaluate our solution with respect to the comms performance in several challenging underground environments including the DARPA SubT Finals competition environment. Our findings support the use of data stratification and flow control to improve bandwidth-usage.

==> Comm and comm-aware autonomy in subt envs_arxiv/results_summary.tex <==
\begin{table}
    \centering
    \caption{Summary of Results}
    \begin{tabular}{c|c|c|c|c}
         & Field Test & Day 1 & Day 2 & Day 3 \\
        \hline \hline
        Time exploring (mins) & 60 & 30 & 30 & 60 \\
        \hline
        Exploring robots (\#) & 6 & 6 & 4 & 6 \\
        \hline
        Deployed radios (\#) & 13 & 1 & 6 & 7 \\
        \hline
        Maximum delay (sec) & 813 & 49 & 1058 & 98 \\
        \hline
        Effective comm range (m) & 173 & 70 & 86 & 68 \\
        \hline
        % \added{\# Critical Messages Dropped} & & & & \\     
        % \hline
        Up time (mins) & 16 & 14 & 20 & 47\\  
        \hline
        % \added{coverage ($\%$)} & & & & \\
        % \hline
        % Max hops (\#) & & & & \\
        % \hline
        Peak data rate & 22.61 & 19.60 & 34.58 & 19.39 \\
        Base $\rightarrow$ Robots (Mbps) & & & & \\
        \hline        
        Peak data rate & 12.43 & 14.41 & 17.14 & 20.30 \\
        Robots $\rightarrow$ Base (Mbps) & & & & \\
    \end{tabular}
    \vspace{-0.0cm}
    \label{tab:results}
\end{table}

% %
% Metrics
% \begin{itemize}
%     \item Time spent exploring
%     \item number of robots supported
%     \item number of radios deployed (and their signal strength)
%     \item time with and without connectivity
%     \item distance traveled before connectivity lost
%     \item time to transfer all data after connectivity is restored
%     \item data rates
%     \item signal strength maps
% \end{itemize}

%%%%%%%%%%%% Final
% Spot 1 - Final
% After filtering for  OK :  320 / 407 (0.786)
% After filtering for  WARN :  59 / 407 (0.1449)
% After filtering for  ERROR :  28 / 407 (0.068)
% After filtering for  FATAL :  0 / 407

% Spot 3 - Final
% After filtering for  OK :  363 / 363 (1.0)
% After filtering for  WARN :  0 / 363
% After filtering for  ERROR :  0 / 363
% After filtering for  FATAL :  0 / 363

% Spot 4 - Final
% After filtering for  OK :  429 / 924 (0.464)
% After filtering for  WARN :  0 / 924
% After filtering for  ERROR :  26 / 924
% After filtering for  FATAL :  469 / 924

% Husky2 - Final
% After filtering for  OK :  315 / 411 (0.766)
% After filtering for  WARN :  0 / 411
% After filtering for  ERROR :  96 / 411
% After filtering for  FATAL :  0 / 411

% Husky3 - Final
% After filtering for  OK :  1117 / 1237 (0.902)
% After filtering for  WARN :  0 / 1237
% After filtering for  ERROR :  120 / 1237
% After filtering for  FATAL :  0 / 1237

%%%%%%%%%%%%% Prelim2
% Spot 1 - Prelim2
% After filtering for  OK :  555 / 614 (0.90)
% After filtering for  WARN :  20 / 614
% After filtering for  ERROR :  39 / 614
% After filtering for  FATAL :  0 / 614

% Spot 3 - Prelim2
% After filtering for  OK :  156 / 839 (0.1859)
% After filtering for  WARN :  376 / 839
% After filtering for  ERROR :  307 / 839
% After filtering for  FATAL :  0 / 839

% Spot 4 - Prelim2
% After filtering for  OK :  412 / 727 (0.5667)
% After filtering for  WARN :  60 / 727
% After filtering for  ERROR :  255 / 727
% After filtering for  FATAL :  0 / 727


% Husky3 -  Prelim2
% After filtering for  OK :  717 / 749 (0.957)
% After filtering for  WARN :  0 / 749
% After filtering for  ERROR :  32 / 749
% After filtering for  FATAL :  0 / 749


%%%%%%%%%%%%% Prelim1 (0.452)
% Spot 1 - Prelim1
% After filtering for  OK :  376 / 718 (0.523)
% After filtering for  WARN :  92 / 718 (0.128)
% After filtering for  ERROR :  250 / 718
% After filtering for  FATAL :  0 / 718

% Spot 3 - Prelim1
% After filtering for  OK :  156 / 839 (0.186)
% After filtering for  WARN :  376 / 839
% After filtering for  ERROR :  307 / 839
% After filtering for  FATAL :  0 / 839

% Spot 4 - Prelim1
% After filtering for  OK :  412 / 727 (0.566)
% After filtering for  WARN :  60 / 727
% After filtering for  ERROR :  255 / 727
% After filtering for  FATAL :  0 / 727

% Husky1 - Prelim1
% After filtering for  OK :  333 / 786 (0.423)
% After filtering for  WARN :  148 / 786
% After filtering for  ERROR :  305 / 786
% After filtering for  FATAL :  0 / 786

% Husky2 - Prelim1
% After filtering for  OK :  489 / 592 (0.826)
% After filtering for  WARN :  66 / 592
% After filtering for  ERROR :  37 / 592
% After filtering for  FATAL :  0 / 592

% Husky3 - Prelim1
% After filtering for  OK :  186 / 967 (0.192)
% After filtering for  WARN :  412 / 967
% After filtering for  ERROR :  369 / 967
% After filtering for  FATAL :  0 / 967


% KY underground Day18 Game 4 (0.264)
% Husky1 - Day18 Game 4
% After filtering for  OK :  268 / 737 (0.363)
% After filtering for  WARN :  0 / 737
% After filtering for  ERROR :  169 / 737
% After filtering for  FATAL :  300 / 737

% Husky2 - Day18 Game 4
% After filtering for  OK :  274 / 1510 (0.181)
% After filtering for  WARN :  16 / 1510
% After filtering for  ERROR :  808 / 1510
% After filtering for  FATAL :  412 / 1510

% Husky3 - Day18 Game 4
% After filtering for  OK :  261 / 1044 (0.25)
% After filtering for  WARN :  0 / 1044
% After filtering for  ERROR :  94 / 1044
% After filtering for  FATAL :  689 / 1044
